Effective Techniques for Message Reduction and Load Balancing in Distributed Graph Computation

Massive graphs, such as online social networks and communication networks, have become common today. To efficiently analyze such large graphs, many distributed graph computing systems have been developed. These systems employ the "think like a vertex" programming paradigm, where a program proceeds in iterations and at each iteration, vertices exchange messages with each other. However, using Pregel's simple message passing mechanism, some vertices may send/receive significantly more messages than others due to either the high degree of these vertices or the logic of the algorithm used. This forms the communication bottleneck and leads to imbalanced workload among machines in the cluster. In this paper, we propose two effective message reduction techniques: (1)vertex mirroring with message combining, and (2)an additional request-respond API. These techniques not only reduce the total number of messages exchanged through the network, but also bound the number of messages sent/received by any single vertex. We theoretically analyze the effectiveness of our techniques, and implement them on top of our open-source Pregel implementation called Pregel+. Our experiments on various large real graphs demonstrate that our message reduction techniques significantly improve the performance of distributed graph computation.

==> system.tex <==
\section{Overview of the Basic Pregel+ System}   \label{sec:system}
We now give an overview of the Pregel+ system, on which we implement our two message reduction techniques. In this section, we only describe the basic vertex-centric framework of Pregel+. We present the system extensions to support effective message reduction in Sections~\ref{sec:mirror} and~\ref{sec:req}.

We use the term ``worker'' to represent a computing unit, which can be a machine or a thread/process in a machine. For ease of discussion, we assume that each machine runs only one worker but the concepts can be straightforwardly generalized.

\subsection{Communication Framework of Pregel+}\label{ssec:communication}
In Pregel+, each worker is simply an MPI (Message Passing Interface) process and communications among different processes are implemented using MPI's communication primitives. Each worker maintains a \emph{message channel}, $Ch_{msg}$, for exchanging the vertex-to-vertex messages. In the {\em compute}() function, if a vertex sends a message $msg$ to a target vertex $v_{tgt}$, the message is simply inserted into $Ch_{msg}$. Like in Google's Pregel, messages in $Ch_{msg}$ are sent to the target workers in batch before the next superstep begins. Note that if a message $msg$ is sent from worker $M_i$ to vertex $v_{tgt}$ in worker $M_j$, the ID of the target $v_{tgt}$ should be sent along with $msg$, so that when $M_j$ receives $msg$, it knows which vertex $msg$ should be directed to.

The operation of the message channel $Ch_{msg}$ is directly related to the communication cost and hence affects the overall performance of the system. We tested different ways of implementing $Ch_{msg}$, and the most efficient one is presented in Figure~\ref{worker}. We assume that a worker maintains $N$ vertices, $\{v_1, v_2,$ $\ldots, v_N\}$. The message channel $Ch_{msg}$ associates each vertex $v_i$ with an incoming message buffer $I_i$. When an incoming message $msg_1$ directed to vertex $v_i$ arrives, $Ch_{msg}$ looks up a hash table $T_{in}$ for the incoming message buffer $I_i$ using $v_i$'s ID. It then appends $msg_1$ to the end of $I_i$. The lookup table $T_{in}$ is static unless graph mutation occurs, in which case updates to $T_{in}$ may be required. Once all incoming messages are processed, {\em compute}() is called for each active vertex $v_i$ with the messages in $I_i$ as the input.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\columnwidth]{worker}
    \vspace{-1mm}
        \caption{Illustration of Message Channel, $Ch_{msg}$}\label{worker}
    \vspace{-3mm}
\end{figure}

A worker also maintains $M$ \emph{outgoing message buffers} (where $M$ is the number of machines), one for each worker $M_j$ in the cluster, denoted by $O_j$. In {\em compute}(), a vertex $v_i$ may send a message $msg_2$ to another vertex with ID $tgt$. Let $hash(.)$ be the hash function that computes the worker ID of a vertex from its vertex ID, then the target vertex is in machine $M_{hash(tgt)}$. Thus, $msg_2$ (along with $tgt$) is appended to the end of the buffer $O_{hash(tgt)}$. Messages in each buffer $O_j$ are sent to worker $M_j$ in batch. If a combiner is used, the messages in a buffer $O_j$ are first grouped (sorted) by target vertex IDs, and messages in each group are combined into one message using the combiner logic before sending.

We also tried other options of implementing $Ch_{msg}$, such as implementing $O_j$ as a hash table with target vertex ID $tgt$ as the key and the set of messages (or the currently combined message) directed to $tgt$ as the value. We find that the implementation described in Figure~\ref{worker} is consistently the most efficient one for various computing tasks over various large real graphs.

\subsection{Comparison with States-of-the-Arts}\label{ssec:why}
{\bf Why implementing the message reduction techniques on Pregel+?\ }\ While the basic vertex-to-vertex messages are exchanged through $Ch_{msg}$ (with combiner properly applied), messages exchanged by our two message reduction techniques are though two other message channels, $Ch_{mir}$ and $Ch_{req}$, which will be described in the next two sections. Therefore, if $Ch_{msg}$ is implemented to be slow, the performance improvement of $Ch_{mir}$ and $Ch_{req}$ would be exaggerated. To fairly evaluate the benefits of our message reduction techniques, they should be implemented on top of a Pregel-like system with a reasonably fast $Ch_{msg}$.

Many studies have compared the performance of existing graph-parallel systems recently~\cite{gSysComp,sys_vldb,sys_sigmod1,sys_sigmod2,guo2013well,sys_bigdata}, including the state-of-the-arts like Pregel+~\cite{ppa_vldb}, Giraph~\cite{giraph}, GraphLab~\cite{graphlab} and GPS~\cite{gps}. \cite{gSysComp} shows that Pregel+ (where messages are passed only through $Ch_{msg}$) is consistently more efficient than Giraph and GraphLab, which implies that Pregel+ is a reasonable choice for implementing and evaluating our message reduction techniques. Neither Pregel+ nor GPS can beat each other in all algorithms on all datasets, but we choose Pregel+ instead of GPS because of the following reason: to avoid the complicated interaction between vertex mirroring and message combining, GPS simply does not perform sender-side message combining, and thus, it is not representative of a typical Pregel-like system.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{btc_gps}
    \vspace{-1mm}
        \caption{Message \# of Each Worker: Hash-Min on BTC in GPS}\label{btc_gps}
    \vspace{-3mm}
\end{figure}

We ran Hash-Min on {\em BTC} in GPS, the results of which are presented in Figure~\ref{btc_gps}, where the taller blue bars (the short red bars) indicate the total number of messages sent by each worker when GPS's LALP optimization is disabled (enabled by mirroring all vertices with degree at least 100)\footnote{We extend GPS to count the number of messages, and the updated codes are accessible from \url{https://github.com/pregel-like/gps}}. Compared with the results of Pregel+ shown in Figure~\ref{msgNum_btc}, GPS sends many more messages per worker as message combining is not used; moreover, the effect of GPS's LALP is not as significant as Pregel+'s optimization that uses both vertex mirroring and message combining, which demonstrates the necessity of applying both techniques.

However, it is amazing that GPS is not much worse in most cases, and is sometimes even faster than Pregel+, even though more messages are exchanged. We studied the codes of GPS to explore the reason, which we explain below. GPS require that the vertex IDs should be integers that are contiguous starting from $0, \cdots, |V|$,\footnote{\url{https://sites.google.com/site/gpsdocumentation/home/input-graph-format}} while other systems allow the vertex IDs to be of any user-specified type as long as a hash function is provided (for calculating the ID of the worker that each vertex resides in). As a result of the dense ID representation, each worker in GPS simply maintains the incoming message buffers of the vertices by an array, and when a worker receives a message targeted at vertex $tgt$, it is put into $tgt$'s incoming message buffer (i.e., $I_{tgt}$) whose position in the array can be directly computed from $tgt$. On the other hand, systems like Pregel+ and Giraph need to look up $I_{tgt}$ from a hash table using key $tgt$, and the cost is required for each message exchanged.

We remark that it is necessary to allow the vertex IDs to take arbitrary type, rather than to hard-code them as contiguous integers. For example, the Pregel algorithm of~\cite{ppa_vldb} for computing bi-connected components constructs an auxiliary graph from the input graph, and each vertex of the auxiliary graph corresponds to an edge $(u, v)$ of the input graph. In this case, using integer pair as vertex ID saves the effort of relabeling the vertices of the auxiliary graph using integer IDs. Although we can easily implement the same message passing mechanism of GPS in Pregel+ to enjoy the better performance when vertex IDs are contiguous integers, it is out of the scope of this paper which studies message reduction techniques for a general Pregel program.

